Optimal Bidding Strategy without Exploration in Real-time Bidding

Maximizing utility with a budget constraint is the primary goal for advertisers in real-time bidding (RTB) systems. The policy maximizing the utility is referred to as the optimal bidding strategy. Earlier works on optimal bidding strategy apply model-based batch reinforcement learning methods which can not generalize to unknown budget and time constraint. Further, the advertiser observes a censored market price which makes direct evaluation infeasible on batch test datasets. Previous works ignore the losing auctions to alleviate the difficulty with censored states; thus significantly modifying the test distribution. We address the challenge of lacking a clear evaluation procedure as well as the error propagated through batch reinforcement learning methods in RTB systems. We exploit two conditional independence structures in the sequential bidding process that allow us to propose a novel practical framework using the maximum entropy principle to imitate the behavior of the true distribution observed in real-time traffic. Moreover, the framework allows us to train a model that can generalize to the unseen budget conditions than limit only to those observed in history. We compare our methods on two real-world RTB datasets with several baselines and demonstrate significantly improved performance under various budget settings.

==> idf.tex <==
What is the problem you are trying to solve? 
  
In programmatic advertising, real-time bidding (RTB) is the typical way ad slots are sold in Ad Exchanges. The main goal of the advertisers, as well as the demand-side platform (DSP), is to devise an optimal bidding strategy such that it maximizes some utility (such as impressions, clicks) with a budget constraint within a time frame. For example, when an advertiser has less money with much time remaining, it might bid low and try to get many low-cost impressions increasing utility whereas when the advertiser has a lot of budgets left with relatively less time, it might try to bid higher aggressively to maximize its utility. The problem falls under the reinforcement learning framework. However, DSP learns a bidding strategy from historical datasets in an offline process without online interaction with the market. Further, DSP does only observe partially some state of the market; for example, DSP knows market price only when it wins the auction. Thus learning from historical datasets with partially observed censored datasets poses few challenges; i) Without exploration, extrapolation error increases. For example, under a new budget constraint, DSP would not have any idea what values to bid. Thus generalization new state space is infeasible with historical datasets. ii) There is no clear evaluation procedure to test any bidding strategy. As the states are partially observed, the only way to test is to pick those points where states were all observed. This leads to a very different distribution than DSP observes in real-time systems.  
Hence to devise a framework such that one can evaluate any bidding strategy as well as learn a model that can generalize to the new budget and time constraint is of utmost importance. This will give DSP a knob through which it can determine the efficiency of any model as well as train a robust model that has generalization property, thereby helping in budget pacing, bidding strategy and optimization. 
  
This invention disclosure outlines a framework that can accurately represent the actual testing environment as seen by the DSP so that the true evaluation metric can be computed. Further, this invention disclosure outlines the framework that can train a model under censored states with generalization property to new state space. We have implemented the framework in public as well as Ad Cloud datasets with positive results. 
  
  
  
How are other people solving the problem?* 
In a real-world application, often the bidding system employs a simple linear bidding strategy [1] where advertiser bids proportional to their perceived value (using estimated utility) due to its simplicity as well as scalability.  
Recently, in [4], the author proposed to solve the Bellman equation using dynamic programming on a simplified learned model. The solution has an attractive property of computing the optimal strategy when the model is correct. However, to tackle large continuous state and action space RLB model assumes market price, as well as the winning rate, is independent of the ad requests. 
Further, to compute optimal action, the optimal strategy 
needs to backtrack in the dynamic programming solution which results in O(k) complexity for each bid request as well as O(T 
2k) memory requirement (T, k is the maximum number of time steps left and the number of bid values respectively). This is unacceptable in the real world situation. The author proposed to use a segmented time window with neural network approximation to the solution of dynamic programming [2] which leads to further approximation in addition to the model simplification. Further, these model-based reinforcement learning algorithms do not generally have the opportunity to explore the real environment. Thus, methods based on such historical datasets are prone to extrapolation errors. For example, if the advertiser’s budget increase 
from $100 to $1000, the model would not know how to 
react without exploration 
  
[1] C. Perlich, B. Dalessandro, R. Hook, O. Stitelman, T. Raeder, and F. Provost, Bid optimizing 
and inventory scoring in targeted online advertising, KDD 2012 
  
[2] H. Cai, K. Ren, W. Zhang, K. Malialis, J. Wang, 
Y. Yu, and D. Guo, Real-time bidding by reinforcement learning in display advertising, WSDM 2017 
  
  
What are the key aspects of your invention that we want to be protected? List the elements of your solution that make it unique.* 
  
While model-free online RL algorithms are conceptually appealing, real-time bidding systems are often constrained with the choice of batch reinforcement learning. Most early approaches of optimal bidding strategy can be classified as a form of batch RL 
[4, 2, 17, 11]. However, the single drawback of any batch RL algorithm is that they can not generalize to new state space due to extrapolation error [8]. Without exploration, often it is not feasible to extrapolate new budget settings. Further, a clear evaluation procedure is lacking in the literature of the bidding system due to the nature of the batch data. Advertiser often observes a 
partially observed as well censored states which lead to the test datasets. Thus early methods of optimal bidding strategy truncate the censored/unobserved part of the test datasets which leads to an altogether different distribution than observed in real-time settings. 
  
We address the challenge of lacking clear evaluation 
procedure as well as the error propagated through batch 
RL methods in the real-time bidding system. We proposed a 
novel framework using the maximum entropy principle that 
can approximate the evaluation metric of the real-time 
bidding system. Further, the framework allows us to train any model-free RL algorithms that can generalize to state space. We compare our methods on real-world public RTB datasets with several baselines and show that our methods improve earlier state-of-the art performance significantly. Additionally, we compare our methods on one of the largest demand-side platforms achieving significant improvement.  
  
  
Given this the key aspects of the invention are as follows: 
  
1. We learn the Market state as well the reward distribution DSP observes through maximum entropy formulation (a form of inverse reinforcement learning where we would like to learn the policy of an expert) 
  
2. Novel Evaluation Framework under Censored and partially observed states that can approximate the true testing environment. 
  
3. Novel learning framework using the Market as well as the DSP state samplers to run any forward reinforcement learning that can interact with the environment.  
  
  
  
Describe technical details of your solution to solve the problem.* 
  
The existing method removes samples with an unobserved state from the test dataset. This makes the evaluation measure biased (towards the bid request that won the auction). Further, existing methods can not explore to handle extrapolation error. 
  
First, we build an inverse reinforcement learning formulation of the market state representation as to the reward trajectory DSP observes. The key idea is that the Market (other DSP, ad exchange, user) acts rationally and can be seen as a trajectory of optimal or near-optimal behavior. Thus using IRL we learn market state representation and reward distribution. Further, we exploit the fact, given current DSP and market state, future market and DSP states are conditionally independent. Thus we can learn any training or testing environment using the Market and reward samplers. Given the samplers and augmented DSP states, we use a model-free RL algorithm to train with exploration that can generalize to new state space. Further, the market model learned from the test dataset allows us to evaluate any bidding strategy. 
  
The existing methods either use a censored regression-based approach or decision tree on top of survival analysis based methods. 
  
The details of the method can be gleaned from Page 3, in the Methodology section of the attached paper. 
  
  
  
What are the advantages of your solution over the prior art?* 
  
  
  
The main advantages of our solution are as follows: 
  
1. More accurate evaluation measures using the learned test market environment.  
  
2. A scalable method, since RLB can learn only a small scale and for large scale segmentation as well as neural approximation is needed. 
  
3. Our methods can be run on a lot of features attributes while inference is fast.  
  
4. Explored model-free RL algorithms using market model generalize better to new state space.  
  
  
  
 
 
